AsterX: a new open-source GPU-accelerated GRMHD code for dynamical spacetimes

We present AsterX, a novel open-source, modular, GPU-accelerated, fully general relativistic magnetohydrodynamic (GRMHD) code designed for dynamic spacetimes in 3D Cartesian coordinates, and tailored for exascale computing. We utilize block-structured adaptive mesh refinement (AMR) through CarpetX, the new driver for the Einstein Toolkit, which is built on AMReX, a software framework for massively parallel applications. AsterX employs the Valencia formulation for GRMHD, coupled with the Z4c formalism for spacetime evolution, while incorporating high resolution shock capturing schemes to accurately handle the hydrodynamics. AsterX has undergone rigorous testing in both static and dynamic spacetime, demonstrating remarkable accuracy and agreement with other codes in literature. Using subcycling in time, we find an overall performance gain of factor 2.5 to 4.5. Benchmarking the code through scaling tests on OLCF's Frontier supercomputer, we demonstrate a weak scaling efficiency of about 67%-77% on 4096 nodes compared to an 8-node performance.

==> figures/workflow.tex <==
\tikzstyle{cell_centered} = [
  rectangle,
  rounded corners,
  minimum width=1cm,
  minimum height=1cm,
  text centered,
  align=center,
  draw=black,
  fill=blue!20
]

\tikzstyle{cell_faces} = [
  rectangle,
  rounded corners,
  minimum width=1cm,
  minimum height=1cm,
  text centered,
  align=center,
  draw=black,
  fill=orange!20
]

\tikzstyle{cell_avg} = [
  rectangle,
  rounded corners,
  minimum width=1cm,
  minimum height=1cm,
  text centered,
  align=center,
  draw=black,
  fill=green!15
]

\tikzstyle{vertex_centered} = [
  rectangle,
  rounded corners,
  minimum width=1cm,
  minimum height=1cm,
  text centered,
  align=center,
  draw=black,
  fill=red!15
]

\tikzstyle{condition} = [
  diamond,
  minimum width=3cm,
  minimum height=1cm,
  text centered,
  align=center,
  draw=black,
  fill=black!30
]

\tikzstyle{infra} = [
  rectangle,
  rounded corners,
  minimum width=3cm,
  minimum height=1cm,
  text centered,
  align=center,
  draw=black,
  fill=black!8
]

\tikzstyle{box} = [
  rectangle,
  rounded corners,
  minimum width=3cm,
  minimum height=1cm,
  text centered,
  align=center,
  inner sep=10pt,
  dashed
]

\tikzstyle{arrow} = [-Latex, line width = 1.5pt]
\begin{figure}
\centering
%\includegraphics[width=0.4\linewidth]
\resizebox{1.1\linewidth}{!}{%
\begin{tikzpicture}[node distance=2cm]

% row 1
\node (eos) [infra] {Equation Of State};
\node (c2p) [cell_avg, below = \singlespace of eos] {$\mbox{\texttt{con2prim}}\left[ \mathbf{F}^0(\mathbf{U}) \right]$};

% row 2
\node (u_cc) [cell_avg, below = \singlespace of c2p] {$\mathbf{U}$ on cell centers};

% row 3
\node(recon) [infra, below = \singlespace of u_cc] {Reconstruction};
\node (llg) [vertex_centered, right = \doublespace of recon] {$\gamma_{ij}$};
\node (shift) [vertex_centered, right = \singlespace of llg] {$\beta^i$};
\node(einstein_rhs) [infra, right = \singlespace of shift] {Einstein's Eqs. RHS};
\node(t_munu) [vertex_centered, right = \singlespace of einstein_rhs] {$T_{\mu\nu}$};

% row 4
\node(u_cell_faces) [cell_avg, below = \singlespace of recon] {$\mathbf{U}$ on cell faces};
\node(g_munu) [vertex_centered, below = \singlespace of llg] {$g_{\mu \nu}$};
\node (lapse) [vertex_centered, right = \singlespace of g_munu] {$\alpha$};

% row 5
\node(riemman_solver) [infra, below = \singlespace of u_cell_faces] {Approximate\\Riemman Solver};
\node(source)[cell_avg, below = \singlespace of lapse] {$\mathbf{S}(\mathbf{U})$};
\node(chris) [vertex_centered, below = \singlespace of g_munu] {$\Gamma^\mu_{\nu\rho}$};

% row 6
\node(fluxes) [cell_avg, below = \singlespace of riemman_solver] {Net $\mathbf{F}^{(i)}(\mathbf{U})$};

% row 7
\node(rhs) [cell_avg, below = \singlespace of fluxes] {RHS:\\$\sqrt{-g}\,\mathbf{S}(\mathbf{U}) - \partial_i\left[ \sqrt{-g}\, \mathbf{F}^{(i)}(\mathbf{U}) \right]$};

% Hydro flow
\draw [color = blue!60, arrow] (eos) -- (c2p);
\draw [color = blue!60, arrow] (c2p) -- (u_cc);
\draw [color = blue!60, arrow] (u_cc) -- (recon);
\draw[color = red!60, arrow] (u_cc) -| (einstein_rhs);
\draw[color = red!60, arrow] (u_cc) -| (t_munu);
\draw [color = blue!60, arrow] (recon) -- (u_cell_faces);
\draw [color = blue!60, arrow] (u_cell_faces) -- (riemman_solver);
\draw [color = blue!60, arrow] (riemman_solver) -- (fluxes);
\draw [color = blue!60, arrow] (fluxes) -- (rhs);
%\draw [color = blue, arrow] (rhs) -- (time_step);

% 3 metric
\draw [color = blue!60, arrow] (llg) -- (g_munu);
\coordinate[above = \singlespace of einstein_rhs] (p0);
\draw[color = red!60, arrow] (llg) |- (p0) -| (einstein_rhs);

% Shift
\draw[color = blue!60, arrow] (shift) -- (g_munu);
\draw[color = red!60, arrow] (shift) -- (einstein_rhs);

% Lapse
\draw[color = blue!60, arrow] (lapse) -- (g_munu);
\coordinate[below = \singlespace of einstein_rhs] (p1);
\draw[color = red!60, arrow] (lapse) -| (p1) -- (einstein_rhs);

% g_{\mu \nu}
\draw[color = blue!60, arrow] (g_munu) -- (chris);
\draw[color = blue!60, arrow] (g_munu) -- (source);
\draw[color = blue!60, arrow] (g_munu) -- (riemman_solver);

% Chris
\draw[color = blue!60, arrow] (chris) -- (source);

% T_munu
\draw[color = red!60, arrow] (t_munu) -- (einstein_rhs);
\coordinate[below = \singlespace of source] (p2);
\draw[color = blue!60, arrow] (t_munu) |- (p2) -- (source);

% Source
\draw[color = blue!60, arrow] (source) -- (rhs);

\end{tikzpicture}
}
\caption{Overview of the AsterX workflow.}
\label{fig:asterx_workflow}
\end{figure}
